Practical Interpolation for Spectrum Cartography through Local Path Loss Modeling

A fundamental building block for supporting better utilization of radio spectrum involves predicting the impact that an emitter will have at different geographic locations. To this end, fixed sensors can be deployed to spatially sample the RF environment over an area of interest, with interpolation methods used to infer received power at locations between sensors. This paper describes a radio map interpolation method that exploits the known properties of most path loss models, with the aim of minimizing the RMS errors in predicted dB-power. We show that the results come very close to those for ideal Simple Kriging. Moreover, the method is simpler in terms of real-time computation by the network and it requires no knowledge of the spatial correlation of shadow fading. Our analysis of the method is general, but we exemplify it for a specific network geometry, comprising a grid-like pattern of sensors. We also provide comparisons to other widely used interpolation methods.

==> estError.tex <==
\section{PL Estimation Error Analysis}
\label{sec:estError}
We have proposed the path loss estimation algorithm in two parts - (1) estimation of $A^"$ and $\gamma$ and (2) interpolation of measured $s^"$-values, each of which attempts to minimize estimation error separately. But these two errors interact and affect each other. In this section, we analyze and quantify each error by itself and their combined effects.

\subsection{Estimation of $A"$ and $\gamma$}
\label{subsec:deltaM}
We assume that the $S_0$-value at the arbitrary point $P_0$ is known. Thus, the only path loss estimation error at $P_0$ is due to imperfect estimations of $A^"$ and $\gamma$. The study of such an artificial situation enables us to characterize the impact of undersampling in estimating $A^"$ and $\gamma$. We quantify this error as $\delta_m$, which is the deviation of estimated median PL from the actual one and given as
\begin{equation}
\label{eq:delm_1}
\delta_{m,0} = \Delta A + 10\Delta\gamma\log d_0.
\end{equation}
where $\Delta A = A^" - A^{'}$, $\Delta\gamma = \gamma - \gamma^{'}$ and $d_0$ is the distance between the emitter and $P_0$.  
To obtain $\Delta A$ and $\Delta\gamma$, we solve for $A^{'}$ and $\gamma^{'}$ by using LSE Eq.~\ref{eq:funAprx}. Using Eq.(\ref{eq:lo_PL}) and rearranging terms, we have\footnote{For the convenience, base 10 is dropped from $\log$ here and for rest of the paper. But please as $\log_10$ wherever $\log$ is appeared.}
\begin{equation}
\label{eq:delm_2}
\begin{aligned}
\delta_{m,0} = \log d_0 \sum_{i=1}^{n}\alpha_{i} S_i + \sum_{i=1}^{n}\beta_{i} S_i,
\end{aligned}
\end{equation}
where
\begin{equation}
\label{eq:delm_2}
\begin{aligned}
&\alpha_i = \frac{\left(\sum_{j=1}^n \log d_j\right) - n\log d_i}
{n\sum_{j=1}^{n}\left(\log d_j\right)^2 - \left(\sum_{j=1}^n\log d_j\right)^2};\\
&\beta_i = \frac{\left(\log d_i\right)\left(\sum_{j=1}^n\log d_j\right) - (1/n)\left(\sum_{j=1}^n\log d_j\right)^2}
{n\sum_{j=1}^{n}\left(\log d_j\right)^2 - \left(\sum_{j=1}^n\log d_j\right)^2}.
\end{aligned}
\end{equation}
It is clear that $\delta_{m,0}$ is a linear sum of shadow-fading $S_i$ at sensors with constant coefficients. Therefore, $\delta_{m,0}$ is a zero-mean Gaussian random variable with derivable value of RMS error. We note that the constant coefficients are functions of emitter-$P_0$ and emitter-sensor distances. Thus, the emitter-sensors-$P_0$ geometry influences the RMS error.

\subsection{Estimation of $S_0^"$ at any arbitrary point $P_0$}
\label{subsec:deltaS}
From Eqs.~\ref{eq:lo_PL}, \ref{eq:sAprx} and \ref{eq:delm_1}, estimate $S^{'}_i$ at sensor $i$ is
\begin{equation}
\label{eq:s_est_i}
S^{'}_i = S^{"}_i + \delta_{m,i}; \forall i.
\end{equation}
and, from Eq.\ref{eq:s5}, estimate of $S_0^"$, is
\begin{equation}
\label{eq:s_est_1}
\begin{aligned}
S^{'}_0 &= \left(\sum_{i=1}^n w_i S^{"}_i\right) + \left(\sum_{i=1}^n w_i\delta_{m,i}\right).
\end{aligned}
\end{equation}

Factors that make $S_0^{'}$ differs from the true value $s_0^"$ are
\subsubsection{Imperfect estimation of $A^"$ and $\gamma$}
Ideally, $S_0^"$ is estimated as a weighted sum over the $\bm{S}^"$ at sensors (as given in the first parenthesis of Eq.~\ref{eq:s_est_1}). Since we only have imperfect values $\bm{S}^{'}$, there will be errors in the estimation of $S_0^"$. 
The the second parenthesis of Eq.~\ref{eq:s_est_1} quantifies the corruption of the $\bm{S}^{'}$ due to errors in $A^"$ and $\gamma$.

\subsubsection{Intractability of Weights}
As discussed earlier, ideal assignment of weights is not available due to the random properties of shadow fading. This contributes to the error in estimating $S_0^"$.
 
\subsubsection{Unavailability of Weights for $\bm{S}^"$}
The proposed path loss estimation algorithm computes $\bm{W}$-vector for $\bm{s}$-values, not for $\bm{s^"}$-values as shown in Eq.~\ref{eq:s_est_1}. As discussed previously, error due to the usage of $s^"$-values is $(\sum_{i=1}^n w_i - 1)Z_n$ (Eq.~\ref{eq:s_55_est}). But this error disappears when $\sum_{i=1}^n = 1$. 
\eat{
Also, as noted earlier in Eq.(\ref{eq:s_55_est}), $(\sum_{i=1}^N w_i - 1)\psi$ is a error part occurs in the proposed local path loss algorithm in which $s^"$-values are used instead of $s$-values.}


\subsection{Total Path Loss Error}
\label{subsec:combinedPLerr}
Combining Eqs. \ref{eq:PL0_est}, \ref{eq:delm_2} and \ref{eq:s_est_1}, the total path loss at the virtual point $P_0$ can be expressed as
\begin{equation}
\label{eq:DeltaPL_0_1}
\begin{aligned}
\Delta PL_0  &= PL_0 - PL^{'}_0\\
&= \left(\delta_{m,0} - \sum_{i=1}^n w_i\delta_{m,i}\right) + \left(S^"_0 - \sum_{i=1}^n w_i S_i\right).
\end{aligned}
\end{equation}
Clearly, first part reflects the total error caused by imperfect estimation of $A^"$ and $\gamma$ and the other part is the error due to unavailability of precise weights. Further solving for $\Delta PL_0$, we have,
\begin{equation}
\label{eq:DeltaPL_0_2}
\begin{aligned}
\Delta PL_0 &= S_0 + \sum_{i=1}^n S_i\left(\alpha_i\log\left(\frac{d_0}{\prod_j d_j^{w_j}}\right) - w_i \right)\\
&+  \sum_{i=1}^n S_i\left(\left(1-\sum_j w_j\right) \left(\beta_i - \frac{1}{n}\right)  \right); j=\{1,..,n\}\\
\end{aligned}
\end{equation}
where $\alpha_i$ and $\beta_i$ are defined by Eq.(\ref{eq:delm_2}). $\Delta PL_0$ is a linear sum of shadow-fading $s_1$ through $s_n$ at sensors and $s_0$ at the virtual point which has coefficients with constant (distance) terms. Therefore, $\Delta PL_0$ can be quantified as a zero-mean Gaussian random variable with derivable RMS error $\Sigma_{\mbox{rms}}$.
